A Conflict-Based Search Framework for Multi-Objective Multi-Agent Path Finding

Conventional multi-agent path planners typically compute an ensemble of paths while optimizing a single objective, such as path length. However, many applications may require multiple objectives, say fuel consumption and completion time, to be simultaneously optimized during planning and these criteria may not be readily compared and sometimes lie in competition with each other. The goal of the problem is thus to find a Pareto-optimal set of solutions instead of a single optimal solution. Naively applying existing multi-objective search algorithms, such as multi-objective A* (MOA*), to multi-agent path finding may prove to be inefficient as the dimensionality of the search space grows exponentially with the number of agents. This article presents an approach named Multi-Objective Conflict-Based Search (MO-CBS) that attempts to address this so-called curse of dimensionality by leveraging prior Conflict-Based Search (CBS), a well-known algorithm for single-objective multi-agent path finding, and principles of dominance from multi-objective optimization literature. We also develop several variants of MO-CBS to improve its performance. We prove that MO-CBS and its variants can compute the entire Pareto-optimal set. Numerical results show that MO-CBS outperforms MOM*, a recently developed state-of-the-art multi-objective multi-agent planner.

==> mosipp.tex <==

\vspace{-1mm}
\subsection{Preliminaries}
We begin with a description about the problem solved by safe-interval path planning (SIPP) and then provide a summary of SIPP.
Given a graph $G=(V,E)$, let $G^t = (V^t, E^t) = G \times \{0,1,\dots,T\}$ denote a time-augmented graph of $G$, where each vertex $v \in V^{t}$ is defined as $v=(u,t), u\in V, t \in \{0,1,\dots,T\}$ and $T$ is a pre-defined time horizon, which is typically a large positive integer. Edges within $G^{t}$ is represented as $E^{t}= V^{t} \times V^{t}$ where $(u_1,t_1),(u_2,t_2)$ is connected in $G^t$ if $(u_1,u_2) \in E$ and $t_2=t_1 + 1$.
Wait in place is also allowed in $G^{t}$ which means $(u,t),(u,t+1), u \in V$ is connected in $G^t$.
A dynamic obstacle with a known trajectory is represented as a set of subsequently occupied nodes in $G^t$.
An illustrative example of $G$, $G^t$ and dynamic obstacles can be found in Fig.~\ref{fig:sipp_eg}.
For the rest of the article, when a node or edge is mentioned, we point out to which graph ($G$ or $G^t$) it belongs if needed.
Given an initial node $v_{init}$ and goal node $v_{goal}$ in $G$, SIPP aims to plan a collision-free trajectory $\tau$ from $v_{init}$ at time zero to $v_{goal}$ with the minimum arrival time.

To solve the problem, A* can be applied to search over $G^t$ to find a collision-free trajectory with the minimum arrival time.
However, this approach is very inefficient as the time dimension is searched in a step-by-step manner.
To overcome this challenge, SIPP~\cite{phillips2011sipp} compresses time steps into intervals.
Let tuple $s=(v,[t_a,t_b])$ denote a search state at node $v\in G$ where $t_a,t_b$ are the beginning and ending time steps of a safe (time) interval respectively.
A safe interval is a maximal contiguous time range in which a node is not occupied by any dynamic obstacles. 
State $s=(v,[t_a,t_b])$ indicates that node $v$ is not occupied by any dynamic obstacle and hence the name safe interval for $[t_a,t_b]$.
Note that, any two safe intervals at the same node never intersect.
Two states are the same, if both states share the same node, beginning time step and ending time step.
Otherwise, two states are different.
Especially, two states with the same node but different safe intervals are different states.
%Based on this definition, given a node $v\in V$ with a finite number of time steps occupied by obstacles, there are a finite number of safe intervals that complement those occupied time steps (Fig.~\ref{fig:sipp_eg}). Assuming a finite number of time steps occupied by obstacles at each node in $G$, the number of the resulting states is finite.

\begin{figure}[htbp]
	\centering
	\includegraphics[width=\linewidth,height=2.3cm]{sipp_eg.png}
	\vspace{-5mm}
	\caption{A toy example of SIPP over a graph $G$ with $6$ (free) nodes.
		The time-augmented graph $G^t$ is visualized with time steps between $0$ and $4$ with edges connecting different time steps omited to make the plot clear.
		A dynamic obstacle enters the environment at node $b$ at time $2$, moves to node $e$ at time $3$ and stays there afterwards.
		At node $b$, there are two possible states $(b,[0,1])$ and $(b, [3,\infty])$ while at node $e$, there is only one possible state $(e,[0,2])$.
		The agent's initial state is $(a,[0,\infty])$.
		To expand it, one successor is generated at node $d$, which is the state $(d,[0,\infty])$ with the earliest arrival time $1$, and two successors are generated at node $b$, which are $(b,[0,1])$ with the earliest arrival time $1$ and $(b, [3,\infty])$ with the earliest arrival time $3$.}
	\label{fig:sipp_eg}
	\vspace{-5mm}
\end{figure}

SIPP conducts A*-like heuristic search.
For each state $s$, let $g(s)$ represent the earliest arrival time at state $s$ at any time of the search and let $h(s)$ denote the heuristic value of $s$, which underestimates the cost-to-goal, i.e. travel time to goal, from $s$.
In addition, the $f$-value of a state is $f(s):=g(s)+h(s)$.
At any time of the search, let OPEN denote the open list containing candidate states to be expanded, where candidate states are prioritized by their $f$-values.

SIPP starts by inserting the initial state $s_o$ into OPEN ($s_o$ is a tuple of $v_{init}$ and the safe interval with a beginning time set to 0).
In each search iteration, a state with the minimum $f$-value in OPEN is popped from OPEN and expanded.
To expand a state $s=(v,[t_a,t_b])$, SIPP considers all reachable successor states from $s$ and finds the earliest possible arrival time onto each of those states via ``wait and move'' action, i.e. wait for an minimum amount of time to arrive at the successor state as early as possible.
An illustration of this expansion process can be found in Fig.~\ref{fig:sipp_eg}.
During the search, SIPP records the so-far earliest arrival time at each state $s$ as $g(s)$.
When a new trajectory is found to reach state $s$ (from $v_{init}$) with an earlier arrival time, $g(s)$ is updated.
Here, a trajectory from $v_{init}$ to some state $s=(v,[t_a,t_b])$ indicates a trajectory from $v_{init}$ to $v$ with an arrival time at $v$ within safe interval $[t_a,t_b]$.
When a state at the goal node (i.e. the node contained in the state is $v_{goal}$) is expanded, a trajectory with the minimum arrival time is found and SIPP terminates.
The key principle behind SIPP can be summarized as follows.
\begin{theorem}\label{thm:sipp}
Arriving at a state $s$ at the earliest possible time can (1) generate the maximum number of successors from $s$ and (2) find the optimal (i.e. minimum arrival time) trajectory from $v_{init}$ to $s$ during the search.
\end{theorem}

We note here that when we introduce SIPP to multi-objective settings in the subsequent sections, this principle needs to be carefully revisited.%only partially holds.

\vspace{-1mm}
\subsection{Multi-objective Problem Formulation}
This section follows the notations and concepts introduced in the previous section.
For a multi-objective trajectory planning problem, let $\vec{c}(e), \forall e\in E^t$ denote a non-negative cost vector associated with edge $e$.
Note that, $E^t$ includes the wait action.
%In this work, we assume that the wait action at any nodes has the same cost vector.
Let $\vec{g}(\tau)$ denote the accumulated cost vector of a trajectory $\tau$, which is the sum of the cost vector of all edges present in $\tau$.
To compare any two trajectories, we compare the cost vectors between them.
Given two vectors $a$ and $b$, $a$ \textit{dominates} $b$ if every component in $a$ is no larger than the corresponding component in $b$ and there exists at least one component in $a$ that is strictly less than the corresponding component in $b$.
Formally, it is defined as follows.
\begin{definition}[Dominance \cite{ehrgott2005multicriteria}]\label{def:dom}
	Given two $M$-dimensional vectors $a$ and $b$, $a$ dominates $b$, notationally $a \succeq b$, if $\forall m \in \{1,2,\dots,M\}$, $a(m) \leq b(m)$, and there exists $m \in \{1,2,\dots,M\}$ such that $a(m) < b(m)$.
\end{definition}
If $a$ does not dominate $b$, we represent this non-dominance as $a \nsucceq b$.
Any two trajectories connecting the same pair of nodes are non-dominated to each other if the corresponding cost vectors do not dominate each other.
%The set of all non-dominated trajectories connecting the start and the goal is called the {\it Pareto-optimal} set.
The goal of the multi-objective trajectory planning problem is to find $\mathcal{T}^*$, a set of all collision-free, non-dominated ($i.e.$ Pareto-optimal) trajectories with unique cost vectors.\footnote{If two trajectories have the same cost vectors, only one of them is kept.}


\vspace{-1mm}
\subsection{Algorithm}\label{sec:mosipp:alg}

As in SIPP, let a search state $s=(v,[t_a,t_b])$ be a tuple of a node and a safe interval.
In SIPP, for each closed state $s$, keeping track of just one trajectory from the start to $s$ with minimum arrival time is sufficient to compute an optimal solution to the goal vertex. In a multi-objective problem, however, there can be multiple trajectories with non-dominated cost vectors connecting $v_{init}$ and state $s$ and all of them need to be recorded at $s$ in order to compute a set of cost-unique Pareto-optimal trajectories $\mathcal{T}^*$ to the goal vertex. The algorithm also needs to be able to discriminate between those trajectories that arrive at the same state $s$ with possibly different cost vectors and arrival times.
Based on this observation, let $l=(s,\vec{g}, t_{r})$ denote a \emph{label} at state $s$, which identifies a specific trajectory from $v_{init}$ to $s$ with an arrival time $t_r$ and a cost vector $\vec{g}$.
Additionally, let $\vec{g}(l)$, $t_r(l)$ and $s(l)$ represent the cost vector, arrival time and state associated with label $l$ respectively.
Also, let $v(l)$, $t_a(l)$ and $t_b(l)$ denote the node (in $G$), beginning time and ending time of the safe interval of state $s(l)$ respectively.

As shown in Algorithm \ref{alg:mo_sipp}, multi-objective safe-interval path planning (MO-SIPP) in general has a similar workflow as SIPP (and A*).
The key differences are presented below.

 \begin{algorithm}[tb]
 	\caption{Pseudocode for MO-SIPP}\label{alg:mo_sipp}
 	\small
 	\begin{algorithmic}[1]
 		%
 		\State{$l_o\gets{(s_o,\vec{0},0)}$}
 		\State{add $l_o$ into OPEN}
 		\State{$\alpha(s) \gets \emptyset, \forall s$}
 		\State{add $l_o$ into $\alpha(s_o)$}
 		\State{$\mathcal{T}\gets \emptyset$}
 		\While{OPEN not empty} \Comment{main search loop}
 		\State{$l \gets$ OPEN.pop() }
 		\State{\textbf{if} $v(l)$ is the goal node \textbf{then}}
 		\State{\indent$\tau\gets$\text{Reconstruct($l$)}}
 		\State{\indent add $\tau$ into $\mathcal{T}$}
 		\State{\indent \text{FilterOpen($l$)}}
 		\State{\indent \textbf{continue}}
 		\State{$L_{succ} \gets$ \text{GetSuccessors}($l$) } 
 		\ForAll{$l' \in L_{succ}$ }
 		\State{\textbf{if} \text{LabelDominated($l'$)} \textbf{then}}
 		\State{\indent \textbf{continue}}
 		\State{$f(l') \gets g(l')$ + $h(s(l'))$}
 		\State{parent($l'$) $\gets l$}
 		\State{add $l'$ into OPEN}
 		\EndFor
 		\EndWhile \label{}
 		\State{\textbf{return} $\mathcal{T}$}
 	\end{algorithmic}
 \end{algorithm}
\vspace{-0mm}

\vspace{-1mm}
\subsubsection{Vector valued cost vectors}
Scalar values $g,h,f$ are replaced with corresponding cost vectors in MO-SIPP.
To make the notation clear, we use $\vec{g},\vec{h},\vec{f}$ to denote the cost vectors in MO-SIPP.
Specifically, $\vec{g}$ is associated with labels and it describes the cost-to-come from $v_{init}$.
$\vec{h}$ is defined over states and $\vec{h}(s)$ represents a component-wise underestimate of the cost vector of all non-dominated paths from state $s$ to the goal node.
Finally, $\vec{f}$ is defined over labels and $\vec{f}(l):=\vec{g}(l)+\vec{h}(s(l))$, which underestimates the cost vector of all trajectories connecting the start and the goal via label $l$.

\vspace{-1mm}
\subsubsection{Label expansion}
OPEN contains all candidate labels for further expansion.
In every search iteration, a label with a non-dominated cost vector within OPEN is selected for further expansion.
The expansion step is similar to the expansion in SIPP with the only difference that MO-SIPP expands and generates new labels (rather than states as in SIPP).
Specifically, to expand a label $l$, MO-SIPP considers all the reachable states from state $s(l)$, and then for each reachable state $s'$, the earliest arrival time $t_r'$ and the cost vector $\vec{g}'$ for reaching $s'$ from $s(l)$ is computed.
A successor label $l'=(s',\vec{g}', t_r')$ is then generated.
After expanding a label $l$, a set of successor labels are obtained for comparison.

\vspace{-1mm}
\subsubsection{Label comparison}

The comparison step in MO-SIPP differs from the one in SIPP.
In SIPP, when a new trajectory from $v_{init}$ to state $s$ is found, the $g$-value of this new trajectory and the previously stored $g$-value at $s$ is compared and the smaller value is kept. %, which identifies the best trajectory obtained thus far in the search process from $v_{init}$ to $s$.
In MO-SIPP, multiple non-dominated trajectories, which are represented by labels, need to be tracked at state $s$.
To do so, first, a new type of dominance between labels is defined as follows.
\begin{definition}[Label-dominance]\label{def:label-dom}
	Given two labels $l=(s, \vec{g}, t_r)$ and $l'=(s', \vec{g}', t_r')$ with $s=s'$ (i.e. nodes and safe intervals in both $s$ and $s'$ are the same), if the following two conditions both hold: (i) $\vec{g}\succeq\vec{g}'$ or $\vec{g} = \vec{g}'$, (ii) $t_r \leq t_r'$,
	then we say $l$ \emph{label-dominates} $l'$. Notationally, $l \succeq_l l'$.
\end{definition}
Subscript $l$ in $\succeq_l$ indicates that it's a comparison between labels rather than cost vectors.
Second, let $\alpha(s)$ denote a set of non-dominated labels at state s.
To initialize, $\alpha(s)$ for all states but the initial state are set to an empty set and $\alpha(s_o)$ is set to be a set containing $(s_o, \vec{0}, 0)$ only.
With that in hand, we now introduce the comparison procedure, as shown in Algorithm.~\ref{alg:compare}.
When a new label $l'$ is generated at state $s$ (i.e. $s(l')=s$), it is compared with every label $l \in \alpha(s)$.
If none of the labels in $\alpha(s)$ label-dominates $l'$, then $l'$ is inserted into $\alpha(s)$ and $l'$ is used to filter $\alpha(s)$, which removes all labels $l \in \alpha(s)$ that are label-dominated by $l'$.
By doing so, at any time of the search, $\alpha(s)$ maintains a set of labels at state $s$ with either a non-dominated cost vector or an earlier arrival time.
Finally, if a generated label is not label-dominated, it is inserted into OPEN for further expansion.

\begin{algorithm}[tbp]
	\caption{Pseudocode for LabelDominated($l'$)}\label{alg:compare}
 	\small
	\begin{algorithmic}[1]
		\State{$l'$ is the input label to be compared.}
		\ForAll{$l \in \alpha(s(l'))$}
		\State{\textbf{if} $ l \succ_l l'$ \textbf{then}}
		\State{\indent\Return true \Comment should be discarded}
		\EndFor
		%
		\ForAll{$l \in \alpha(s(l'))$}
		\State{\textbf{if} $ l' \succ_l l$ \textbf{then}}
		\State{\indent remove $l$ from $\alpha(s(l'))$}
		\State{\indent remove $l$ from OPEN if OPEN contains $l$.}
		\EndFor
		\State{add $l'$ to $\alpha(s(l'))$}
		\State{\Return false \Comment should not be discarded}
	\end{algorithmic}
\end{algorithm}
\vspace{-1mm}


\vspace{-1mm}
\subsubsection{Filtering and termination}
During the search, when a label $l$ with $v(l)$ being the goal node is popped from OPEN, a Pareto-optimal trajectory is found and is inserted into $\mathcal{T}$, which is a set that contains all Pareto-optimal trajectories found during the search.
The trajectory represented by a label can be easily reconstructed by iteratively backtracking the parent pointers of labels.
Different from SIPP, what's new in MO-SIPP is that the cost vector $\vec{g}(l)$ is used to filter OPEN, which removes all candidate labels $l'$ in OPEN if $\vec{g}(l) \succeq \vec{g}(l')$ or $\vec{g}(l) = \vec{g}(l')$.
The intuition behind this filtering is that, any filtered candidate labels can not be part of a Pareto-optimal trajectory and is thus discarded, as the cost vectors of all edges in $G^t$ are non-negative.
MO-SIPP terminates when OPEN is empty, which guarantees that $\mathcal{T}$ contains all cost-unique Pareto-optimal trajectories.

\vspace{-1mm}
\subsection{Analysis}
In this section, we show that MO-SIPP is able to compute a set of cost-unique Pareto-optimal trajectories $\mathcal{T}^*$.
%As shown in Theorem \ref{thm:sipp}, SIPP has two key properties. In the proposed MO-SIPP, only the first property holds, which is described by the following lemma.
\begin{lemma}\label{lem:max_succ}
	Arriving at a state $s$ at the earliest possible time can generate the maximum number of successors.
\end{lemma}
\begin{proof} Note that the set of reachable successors from a label corresponding to a state depends only on the arrival time of the label and is not dependent on the cost vector of the label. Therefore, given two labels $l=(s,\vec{g},t_r)$ and $l'=(s,\vec{g}',t'_r)$ at the same state $s=(v,[t_a,t_b])$ with $t_r \leq t'_r$, any reachable state from $l'$ (within time interval $[t'_r,t_b]$) is also reachable from $l$ (within time interval $[t_r,t_b]$), regardless of the cost vectors $\vec{g}$ or $\vec{g}'$. Hence proved.
\end{proof}
\vspace{1mm}

The second property of SIPP  in Theorem  \ref{thm:sipp} does not apply to MO-SIPP because SIPP aims to optimize the arrival time corresponding to a single objective while MO-SIPP aims to find non-dominated trajectories corresponding to multiple objectives. With the modified label comparison procedure in MO-SIPP, the following lemma holds.

\vspace{1mm}
\begin{lemma}\label{lem:dom_prune}
	At any time of the search, if a label at state $s$ is pruned, the trajectory represented by the label cannot be part of a cost-unique Pareto-optimal trajectory.
\end{lemma}
\begin{proof}
In MO-SIPP, there are three cases where a label $l'$ is pruned:
\begin{itemize}
	\item $l'$ is filtered by the FilterOpen procedure;
	\item $l'$ is label-dominated by an existing label $l\in \alpha(s(l'))$ (line 3 in Algorithm~\ref{alg:compare});
	\item $l'$ is label-dominated by a label $l$ that enters $\alpha(s(l'))$  (line 6 in Algorithm~\ref{alg:compare}). 
\end{itemize}
For either of those three cases, $\vec{g}(l')$ is dominated by or equal to the cost vector of some other labels expanded or to be expanded.
In addition, if a label $l'$ is label-dominated by $l$, any possible successors of $l'$ is also reachable from $l$ since $t_r(l) \leq t_r(l')$.
Therefore, $l'$ cannot be part of a cost-unique Pareto-optimal trajectory.
\end{proof}
\vspace{1mm}

Therefore, in MO-SIPP, label expansion always generates successors with the earliest arrival time which guarantees the maximum number of successors (Lemma~\ref{lem:max_succ}).
Those generated successor labels are only pruned if they cannot lead to a cost-unique Pareto-optimal trajectory (Lemma~\ref{lem:dom_prune}).
MO-SIPP terminates when OPEN is empty, which means all labels are expanded or pruned, which computes a $\mathcal{T}^*$. This property can be summarized with the following theorem:

\vspace{1mm}
\begin{theorem}\label{thm:mo_sipp}
	MO-SIPP algorithm is able to compute all cost-unique Pareto-optimal trajectories connecting the start and the goal.
\end{theorem}


==> prior_work.tex <==
\noindent\textbf{Related Work.}
MAPF methods~\cite{luna2011push,wang2008fast,silver2005hca,yu2013structure_nphard,surynek2017sat} range from centralized to decentralized, trading off completeness and optimality for scalability. 
%To name a few, rule-based approaches \cite{luna2011push, de2013pushrotate,wang2008fast}, seek to overcome the curse of dimensionality by resolving agent-agent interaction with pre-defined primitives and compute non-optimal solution with good scalability. Decentralized approaches \cite{vcap2015complete,wiktor2014decentralized,silver2005hca,van2005prioritized}) achieve scalability by decomposing the joint configuration space into a sequence of individual configuration spaces and plan for agents one after another in a pre-defined sequence. %Reduction-based methods reduce MAPF problem to known problems \cite{yu2013structure_nphard,surynek2017sat,ryan2010cop}, who have their own approaches to handle high dimensional search spaces. 
Conflict-based search (CBS)~\cite{sharon2015conflict}, a leading method in the middle of the spectrum, have been improved~\cite{boyarski2015icbs,barer2014suboptimal} and extended to many different problems \cite{Ma2017Lifelong,cohen2019optimal}, to name a few.

%In the middle of the spectrum, Subdimensional Expansion \cite{wagner2015subdimensional} overcomes the curse of dimensionality by dynamically modifying the dimension of the search space based on agent-agent conflicts. This framework is applicable to many algorithms \cite{wagner2012probabilistic,wagner2015subdimensional}, and inherits completeness and optimality, if the underlying algorithm already has these features, while scaling well \emph{on average} in less crowded environments. 

%where on the high level, every agent's path is stored as search information and conflicts between agents' paths are detected. On the low level, constraints derived from those detected conflicts are added to the agent's individual planning space, and new paths are computed obeying constraints are computed to update the high level search information. CBS has been enhanced

%\paragraph{Multi-objective Search}
%However, all the aforementioned MAPF approaches optimize a single scalar-valued objective. 
To optimize multiple objectives, dominance principles from multi-objective optimization (MOO) \cite{ehrgott2005multicriteria} have been applied to single agent path finding \cite{moastar,mandow2008multiobjective,ulloa2020simple}, motion planning~\cite{tesch2013expensive}, reinforcement learning \cite{roijers2013survey} and others \cite{deb2001multi,montoya2013multiobjective}, to name a few.
With respect to MOO for multiple agents, the only work we are aware of is on evolutionary algorithms~\cite{weise2020momapf} for a related variant of MOMAPF considered in this work.
Specifically, in \cite{weise2020momapf}, the conflicts between the agent's paths is modeled in one of the objectives and not as a constraint; as a result, a solution in the Pareto-optimal set may have agent's paths that conflict with each other. In addition, the work in \cite{weise2020momapf} enforces a pre-defined number of waypoints to be visited in the middle of each agent's path and assumes no wait times for agents at any vertex in the graph, which greatly reduces the size of the Pareto-optimal set.
In this work, we allow for agents to wait at any vertex in the graph and seek conflict-free paths for agents in any feasible solution as in the standard MAPF~\cite{stern2019multi}.

One of the basic challenges in multi-objective search is to compute the entire set of Pareto-optimal solutions~\cite{serafini1987some, ehrgott2005multicriteria}.
To overcome this challenge, search algorithms like A*~\cite{astar}, as a best-first search method, are extended to multi-objective A* (MOA*)~\cite{moastar} and later improved in NAMOA*~\cite{mandow2008multiobjective}.
Even though MOA*-based approaches can be applied to the product of the configuration spaces of agents, numerical results in Sec.~\ref{sec:result} show that it is significantly less efficient compared to the proposed MO-CBS.

